Survey on Privacy-Preserving Techniques for Data Publishing

The exponential growth of collected, processed, and shared microdata has given rise to concerns about individuals' privacy. As a result, laws and regulations have emerged to control what organisations do with microdata and how they protect it. Statistical Disclosure Control seeks to reduce the risk of confidential information disclosure by de-identifying them. Such de-identification is guaranteed through privacy-preserving techniques. However, de-identified data usually results in loss of information, with a possible impact on data analysis precision and model predictive performance. The main goal is to protect the individuals' privacy while maintaining the interpretability of the data, i.e. its usefulness. Statistical Disclosure Control is an area that is expanding and needs to be explored since there is still no solution that guarantees optimal privacy and utility. This survey focuses on all steps of the de-identification process. We present existing privacy-preserving techniques used in microdata de-identification, privacy measures suitable for several disclosure types and, information loss and predictive performance measures. In this survey, we discuss the main challenges raised by privacy constraints, describe the main approaches to handle these obstacles, review taxonomies of privacy-preserving techniques, provide a theoretical analysis of existing comparative studies, and raise multiple open issues.

==> A Survey of Data Privacy-Predictive Strategies (1)/tables/data_utility.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{tabular}{@{}ccc@{}}
\toprule
\multicolumn{2}{c}{\textbf{Data utility measures}}                                   & \textbf{Main references}         \\ \midrule
\multicolumn{2}{c}{\multirow{3}{*}{\textbf{Information loss}}}                       &  \citet{bayardo2005data}, \citet{kullback1951information}, \\
\multicolumn{2}{c}{}                                                                 & \citet{machanavajjhala2007diversity}, \citet{samarati2001protecting},                          \\
\multicolumn{2}{c}{}                                                                 & \citet{iyengar2002transforming}, \citet{nergiz2007thoughts}                        \\ \midrule

\multirow{4}{*}{\textbf{Predictive performance}} & \multirow{2}{*}{\textbf{Supervised}}   & \citet{Kent_prec_acc}, \citet{Rijsbergen_fmeasure}, \citet{kubat1998machine},                       \\
                                            &                                        &  \citet{weng2008new}, \citet{iyengar2002transforming}                             \\ \cmidrule(l){2-3} 
                                            & \multirow{2}{*}{\textbf{Unsupervised}} & \citet{rand1971objective}, \citet{davies1979cluster},                             \\
                                            &                                        & \citet{fowlkes1983method}, \citet{rousseeuw1987silhouettes}                              \\ \bottomrule
\end{tabular}

==> A Survey of Data Privacy-Predictive Strategies (1)/tables/ppt_ad.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{tabular}{@{}cll@{}}
\toprule
{\textbf{Privacy-preserving techniques}} & \multicolumn{1}{c}{\textbf{Advantages}}      & \multicolumn{1}{c}{\textbf{Disadvantages}}                                                                                                                     \\ \midrule
\textbf{Non-perturbative}                                                             & \begin{tabular}[c]{@{}l@{}}- Does not disturb data structure;\\ \\ - Unique combinations may disappear. \end{tabular}                                                                                                                               &   \begin{tabular}[c]{@{}l@{}} - Reduces the detail of information;\\ \\ - High generalisation level and many suppressed values \\ destructs data utility.\end{tabular} \\ \midrule

\textbf{Perturbative}                                                                 & \begin{tabular}[c]{@{}l@{}}- Creates uncertainty around the values;\\ \\ - New combinations may appear. \end{tabular}                                                                                                                                                   & \begin{tabular}[c]{@{}l@{}} - It may creates inconsistencies;\\ \\ - Extreme values require great quantity of distortion.\end{tabular}                                                            \\ \midrule
\textbf{De-associative}                                                               & \begin{tabular}[c]{@{}l@{}}- Publishes QIs in their original form;\\ \\ - Breaks the relationship between QIs and \\ sensitive attributes.\end{tabular} 

& \begin{tabular}[c]{@{}l@{}}- Presents high disclosure risk when QIs are the original ones;\\ \\ - The swapped sensitive values could interfere with its true \\ meaning and patterns leading to inaccurate results.\end{tabular}                                                                      \\  \bottomrule
\end{tabular}


==> A Survey of Data Privacy-Predictive Strategies (1)/tables/ppt_summary.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{tabular}{@{}clll@{}}
\toprule
\multicolumn{2}{c}{\textbf{Privacy-preserving techniques}}         & \multicolumn{1}{c}{\textbf{Data type}} & \multicolumn{1}{c}{\textbf{Principle}} \\ \midrule
\multirow{5}{*}{\textbf{Non-perturbative}} & Global recoding       & Both                                       &   Combines several categories to form more general categories.                                     \\
                                           & Local recoding        &  Both           & Recodes into broader categories only some values.                                       \\
                                           & Top-and-bottom coding &   Both                                     &  Replaces values above or bellow of a defined threshold.                                      \\
                                           & Suppression           &  Both          &   Deletes cells/rows/attributes or replace them with special characters.                                     \\
                                           & Sampling      &    Both        &  Selects a sample of the original microdata.                                      \\ \midrule
\multirow{7}{*}{\textbf{Perturbative}}     & Swapping      &   Both                                   &   Exchanges the values of certain attributes across records.                                    \\
                                           & Re-sampling           &   Both         &  Takes independent samples using bootstrap and averages the samples.                                     \\
                                           & Noise        &  Numerical                & Replaces the values by adding/subtracting/multiplicating random values.                                       \\
                                           & Microaggregation      &  Both      &    Groups similar values and assigns an aggregated value to the group.                                    \\
                                           & Rounding           & Numerical          & Replaces values with rounded ones determined by the multiples of a base.                                       \\
                                           & PRAM                  &                  Categorical       &  Reclassifies the values according to the Markov matrix.                                      \\
                                           & Shuffling      & Numerical              &   Uses a regression model to determine which values are exchanged.                                     \\ \midrule
\multirow{4}{*}{\textbf{De-associative}}   & Bucketisation         &           Categorical      &  Bucketises data and permutes the sensitive values.   \\
                                           & Anatomisation         &   Categorical     &   Bucketises data and publishes a QIT and a ST.                                      \\
                                           & Angelisation  &    Categorical   &   Divides data into batches and then buckets, and publishes a BT and a GT.                                     \\
                                           & Slicing     &    Categorical      &   Partitionates data vertically and horizontally.                                     \\ \bottomrule
\end{tabular}

==> A Survey of Data Privacy-Predictive Strategies (1)/tables/risk_measures.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{tabular}{@{}ccccc@{}}
\toprule
\textbf{Disclosure risk}                     & \multicolumn{2}{c}{\textbf{Type}}                                       & \textbf{Privacy risk measures}     & \textbf{QI data type} \\ \midrule
\multirow{25}{*}{\textbf{Identity}}          & \multirow{16}{*}{Uniqueness} & \multirow{2}{*}{Singling out}            & $k$-Anonymity~\cite{samarati2001protecting}             & Categorical           \\ \cmidrule(l){4-5} 
                                             &                              &                                          & $k$-Map~\cite{el2008protecting}                            & Categorical           \\ 
                                            
                   \cmidrule(l){3-5} &                              & \multirow{10}{*}{Probabilistic modelling} & Poisson-gamma~\cite{bethlehem1990disclosure}                      & Categorical           \\ \cmidrule(l){4-5} 
                                             &                              &                                          & Poisson-log-normal~\cite{skinner1998estimating, skinner2002measure}                 & Categorical           \\ \cmidrule(l){4-5} 
                                             &                              &                                          & Ewens~\cite{ewens1990population}                              & Categorical           \\ \cmidrule(l){4-5} 
                                             &                              &                                          & Dirichlet-multinominal~\cite{takemura1999some}             & Categorical           \\ \cmidrule(l){4-5} 
                                             &                              &                                          & Logarithmic series~\cite{hoshino2001applying}                 & Categorical           \\ \cmidrule(l){4-5} 
                                             &                              &                                          & Pitman~\cite{hoshino2001applying}                             & Categorical           \\ \cmidrule(l){4-5} 
                                             &                              &                                          & Gaussian Copulas~\cite{rocher2019estimating}                   & Categorical           \\ \cmidrule(l){3-5} 
                                             &                              & \multirow{2}{*}{Special uniques}         & SUDA~\cite{elliot2002computational}                               & Categorical           \\ \cmidrule(l){4-5} 
                                             &                              &                                          & SUDA2~\cite{manning2008recursive}                              & Categorical           \\ \cmidrule(l){2-5} 
                                             & \multicolumn{2}{c}{\multirow{5}{*}{Outliers}}                           & Rank-based intervals~\cite{mateo2004outlier}               & Numerical             \\ \cmidrule(l){4-5} 
                                             & \multicolumn{2}{c}{}                                                    & Standard deviation-based intervals~\cite{mateo2004outlier, truta2006global} & Numerical             \\ \cmidrule(l){4-5} 
                                             & \multicolumn{2}{c}{}                                                    & Distance-based intervals~\cite{vaidya2004privacy, templ2008robust}           & Numerical             \\ \cmidrule(l){4-5} 
                                             & \multicolumn{2}{c}{}                                                    & Density-based intervals~\cite{foschi2011disclosure}            & Numerical             \\ \cmidrule(l){2-5} 
                                             & \multicolumn{2}{c}{\multirow{2}{*}{Clustering}}                         & Distance-based~\cite{bacher2002re}                     & Numerical             \\ \cmidrule(l){4-5} 
                                             & \multicolumn{2}{c}{}                                                    & Density-based~\cite{ichim2009disclosure}                      & Numerical             \\ \midrule
\multirow{9}{*}{\textbf{Identity/Attribute}} & \multicolumn{2}{c}{\multirow{4}{*}{Record linkage}}                     & Probabilistic-based~\cite{fellegi1969theory, jaro1989advances}                     & Both                  \\ \cmidrule(l){4-5} 
                                             & \multicolumn{2}{c}{}                                                    & Distance-based~\cite{pagliuca1999some, torra2006using}                & Both                  \\ \cmidrule(l){4-5} 
                                             & \multicolumn{2}{c}{}                                                    & Rank-based~\cite{muralidhar2016rank, nin2008rethinking}                         & Both                  \\ \cmidrule(l){2-5} 
                                             & \multicolumn{2}{c}{\multirow{3}{*}{$k$-Anonymity-based}}                &
                $(\alpha, k)$-Anonymity~\cite{wong2006alpha} & Categorical \\
                \cmidrule(l){4-5}
                & 
                \multicolumn{2}{c}{}              & $l$-Diversity~\cite{machanavajjhala2007diversity}                      & Categorical           \\ \cmidrule(l){4-5} 
                                             & \multicolumn{2}{c}{}                                & $(p, k)$-Angelisation~\cite{anjum2018efficient}              & Categorical           \\ \midrule
\multirow{5}{*}{\textbf{Attribute}}          & \multicolumn{2}{c}{\multirow{5}{*}{$k$-Anonymity-based}}                & $(X, Y)$-Anonymity~\cite{wang2006anonymizing}                 & Categorical           \\ \cmidrule(l){4-5} 
                                             & \multicolumn{2}{c}{}                                                    & $t$-Closeness~\cite{li2007t}                      & Categorical           \\ \cmidrule(l){4-5} 
                                             & \multicolumn{2}{c}{}                                                    & $\sigma$-Disclosure privacy~\cite{brickell2008cost}        & Categorical           \\ \cmidrule(l){4-5} 
                                             & \multicolumn{2}{c}{}                                                    & $\beta$-Likeness~\cite{cao2012publishing}                   & Categorical       \\ \bottomrule
\end{tabular}

==> A Survey of Data Privacy-Predictive Strategies (1)/tables/tools.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{tabular}{@{}lccccccc@{}}
\toprule
\textbf{Privacy tool} & \textbf{Open source} & \textbf{Web app} & \textbf{Non-perturbative} & \textbf{Perturbative} & \textbf{De-associative} & \textbf{Privacy assessment} & \textbf{Utility assessment} \\ \midrule
\textbf{$\mu$-ARGUS}  &     \checkmark  &    $x$  &    \checkmark   &  \checkmark  &  $x$   &  \checkmark   &    $x$                   \\
\textbf{UTD}         &     \checkmark       &    $x$     &       \checkmark      &         \checkmark    &   \checkmark   &    \checkmark   &   \checkmark \\
\textbf{Cornell}  &     \checkmark     &    $x$     &   \checkmark  &    $x$     &    $x$   &    \checkmark     &    \checkmark     \\
\textbf{sdcMicro}     &     \checkmark     &   $x$     &   \checkmark    &  \checkmark   &    $x$    &    \checkmark     &  \checkmark   \\
\textbf{ARX}     &    \checkmark    &   $x$  &    \checkmark&     \checkmark      &    $x$    &    \checkmark      &    \checkmark      \\
\textbf{Amnesia}      &   \checkmark      &  \checkmark       & \checkmark       &  $x$    &     $x$  &    \checkmark       &     \checkmark    \\
\textbf{Aircloack}    &   $x$      &    \checkmark     &   \checkmark    &          \checkmark      &   $x$     &    \checkmark       &   \checkmark    \\ \bottomrule
\end{tabular}
